Improving Conversational Recommendation Systems' Quality with Context-Aware Item Meta Information

Conversational recommendation systems (CRS) engage with users by inferring user preferences from dialog history, providing accurate recommendations, and generating appropriate responses. Previous CRSs use knowledge graph (KG) based recommendation modules and integrate KG with language models for response generation. Although KG-based approaches prove effective, two issues remain to be solved. First, KG-based approaches ignore the information in the conversational context but only rely on entity relations and bag of words to recommend items. Second, it requires substantial engineering efforts to maintain KGs that model domain-specific relations, thus leading to less flexibility. In this paper, we propose a simple yet effective architecture comprising a pre-trained language model (PLM) and an item metadata encoder. The encoder learns to map item metadata to embeddings that can reflect the semantic information in the dialog context. The PLM then consumes the semantic-aligned item embeddings together with dialog context to generate high-quality recommendations and responses. Instead of modeling entity relations with KGs, our model reduces engineering complexity by directly converting each item to an embedding. Experimental results on the benchmark dataset ReDial show that our model obtains state-of-the-art results on both recommendation and response generation tasks.

==> approach_12_05.tex <==
The goal of our system is to directly infer user requirements from dialog context and generate accurate recommendations accordingly. Dialog context is represented as a sequence of word tokens ($w_{i,1}, w_{i,2}, ..., w_{i,m}$) where each (i,j) pair denotes the $j_{th}$ token of the $i_{th}$ utterance. Each word token is from either the user looking for items or the system providing recommendations. For each item in our item database, we collect its metadata. For example, in movie recommendation, we collect the title, genre, plots, actors, etc. of each movie. We denote the collected metadata of the entire item database with n items as ($M_1, M_2, ..., M_n$) where each element is subscripted by its index in the database.
% Dialog context is represented as a sequence of utterances ($U_1, U_2, ..., U_l$) where l represents the turn number. Each utterance is from either the user looking for items or the system aiming to generate recommendations. Every utterance $U_i$ is comprised of word token sequence ($w_{i,1}, w_{i,2}, ..., w_{i,m}$) where each (i,j) pair denotes the $j_{th}$ token of the $i_{th}$ utterance. For each item in our item database, we collect its metadata. For example, in movie recommendation, we collect the title, genre, plots, actors, etc. of each movie. We denote the collected metadata of the entire item database with n items as ($M_1, M_2, ..., M_n$) where each item is subscripted by its index in the database.

\subsection{Item Encoder}

Unlike previous works where item representations are constructed based on their connections with other items in the knowledge graph \cite{chen-etal-2019-towards, wang2021finetuning}, we propose to use an item encoder to explicitly map the metadata of each item to an embedding. In movie recommendation, title, genre, actors, directors and plot information are collected and concatenated with a "[SEP]" token for each movie entity appeared in the corpus. This concatenated information is the input to the item encoder. The item encoder consists of a distil-bert \cite{sanh2020distilbert} model that maps the concatenated metadata of each item to a sequence of vectors embeddings, a pooling layer to condense the output of the distil-bert model to a single vector embedding, and a feed-forward neural network layer for additional processing of the embedding. A visualization of this module is shown in Figure \ref{fig:ItemEncoder}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=1.0\columnwidth]{Figures/ItemEncoder.pdf}
    \caption{Item Encoder maps each item to a vector embedding}
    \label{fig:ItemEncoder}
\end{figure}

\subsection{Context Construction}
\label{sec:context}

Previous studies have shown that end-to-end frameworks cannot always integrate the recommended items into the generated replies \cite{wang2021finetuning}. To solve this issue, we replace each item name with a special word token, "[PLACEHOLDER]", in the word sequence. This modified word sequence then gets mapped to a word token embedding (WTE) sequence by the vocabulary embedding matrix of the pre-trained language model. To retain item information, whenever an item i is replaced by the placeholder token, an item token embedding (ITE) with dimension equals the dimension of the WTEs is created by passing the item's metadata through an item encoder, which we refer to as the \textbf{Context Encoder}, and appended to the end of the WTE sequence. In the subsequent tasks, the PLM takes in this entire token embedding sequence as input and aggregates the sequence with other embeddings like positional encodings. The PLM trained on this constructed context aims to generate responses with placeholder tokens to be filled in by the recommended items' names. A visualization of the example is shown in \ref{fig:ContextConstruction}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=1.0\columnwidth]{Figures/ContextConstruction.pdf}
    \caption{Context token embeddings are comprised of both WTEs and ITEs.}
    \label{fig:ContextConstruction}
\end{figure}

\subsection{Recommendation Model}

Similar to \cite{45530}, we pose recommendation as a two phase process: candidate generation and candidate ranking. During candidate generation, the entire item database is traversed and narrowed down to a few hundred candidates based on the dialog context. During candidate ranking, more time-consuming computations can be carried out because only a few hundred items are being considered rather than the entire database. Similarities between the dialog context and the generated candidates are calculated by a PLM and a score is assigned to each candidate in the ranking phase.

\subsubsection{candidate generation}
\label{sec:c_gen}
In this section, we describe the training objective of candidate generation. A light weight method is proposed to train the model to go through the entire database and select candidates relevant to the dialog history. We add a special token "[REC]" to the vocabulary embedding matrix of the PLM. This token serves as the signal to generation recommendations and performs summarization on the dialog context. At the end of each utterance, a dialog context C is created following section \ref{sec:context} in the format of a mixture of word token embeddings (WTE) and item token embeddings (ITE). When recommendation is labeled in a turn in the training dataset, the WTE of "[REC]" is appended to the dialog context C to form an embedding sequence $C'$. Next, the PLM takes in $C'$ and produces an output embedding sequence. We denote the last vector of this output embedding sequence as $O_{[REC]}$ which corresponds to the appended special token [REC] and contains a summarization of all other context tokens in the dialog context.

In order to let the model differentiate between good and bad recommendations, we randomly sample N items and their metadata from the database as negative examples and combine them with the ground truth item labeled in the dataset to get the metadata set. Another item encoder, referred to as the \textbf{candidate encoder} is created to map the metadata set to a set of vector embeddings S = $(s_0, s_1, ..., s_N)$, each with the same dimension as $O_{[REC]}$. The recommendation task at this phase is posed as a multi-class classification problem of predicting the ground truth item over the negative samples. The probability of each candidate item is defined as:

\begin{align}
P(i) = \frac{e^{s_i \cdot O_{[REC]}}}{\sum_{n=0}^{N} e^{s_n \cdot O_{[REC]}} }
\end{align}

For each sample the cross-entropy loss is minimized for the ground truth and the sampled negative items. We denote the loss function of the candidate generation phase as $L_{cg}$.

% During inference time, this classification problem is reduced to a time-efficient top k nearest neighbor search \cite{Liu2004AnIO} over the encoded metadata of the entire item database. In an industry setting, candidate generation often considers multiple sources with both rule-based and neural-network-based filtering methods. To maximize the performance of the model, a rule-based candidate source is also included during inference time. Specifically, whenever an item is mentioned in dialog history during inference phase, we look in the training corpus for all items that appear in the same conversation with that mentioned item and append them to the candidates generated by nearest neighbor search.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=2.1\columnwidth]{Figures/ModelGraphV5.pdf}
    \caption{During training, N and M examples are sampled from the metadata database and participate in computing the joint loss $L_{recall}$ and $Loss_{rank}$. During serving time, the entire metadata DB is stored as a nearest neighbor index (NNI). An approximate nearest neighbor search is performed on $O_{rec}$ to get candidate items, which is then fed to the context encoder to receive scores and be presented to the users in a sorted order.}
    \label{fig:fig1}
\end{figure*}


\subsubsection{candidate ranking}
\label{sec:c_ranking}
In this section, we describe the training objective of candidate ranking. The primary goal of candidate ranking is to perform fine-grained selection on generated candidates so that the final rankings of items can better reflect users' preferences. Unlikely previous studies where knowledge graphs are applied to carry out this task, we propose to use the pre-trained language model. During training, the same concatenated context $C'$ is created for the conversation turn labeled with recommendation. Next, another sampling from the database is done to obtain a set of M negative samples and combined with the ground truth to form a metadata set for ranking training. The \textbf{context encoder} from section \label{sec:context} is used to map the set to an ITE set T = $(t_0, t_1, ..., t_M)$. A concatenation of context $C'$ and T are fed into the same PLM used above and the output embeddings are computed. Note that the order of candidate items should not make a difference on the output scores. Therefore, we add the same positional encoding to each ITE in $T$ and remove the auto-regressive attention masks among the ITE in $T$. We select from the output embeddings the vectors that correspond to the vectors in T. For each output vector selected, a feed-forward layer is applied to reduce each vector from a higher dimension to a single number with dimension equals 1. This set of numbers are denoted by Q = $(q_0, q_1, ..., q_M)$ where the index of each number corresponds to their index in T. The ranking score of each candidate item is defined as:

\begin{align}
R(i) = \frac{e^{q_i}}{\sum_{n=0}^{M} e^{q_n} }
\end{align}

Similar to candidate generation, the cross-entropy loss is minimized for the ground truth and the sampled negative items. We denote the loss function of the candidate ranking phase as $L_{cr}$.

% Pre-trained Models \cite{devlin-etal-2019-bert, lan2020albert, Radford2019gpt2} have proven to have excellent language understanding abilities and have the potential to learn meaningful joint representations under multimodal settings \cite{lu2019vilbert, zhou-etal-2018-visual, li-liang-2021-prefix}. We propose to directly use PLM \cite{Radford2019gpt2} to generate item rankings given the candidates select in \ref{sec:c_gen}. Given dialog context $U_{rec}$ and metadata of candidate items $K = (K_{g_0}, K_{g_1}, K_{g_2}, ..., K_{g_N})$, another encoder, which we refer to as \textbf{Ranking Encoder}, is used to map each $K$ to a vector set  $S = (S_{g_0}, S_{g_1}, S_{g_2}, ..., S_{g_N})$ whose dimensions equal the input word embedding dimension of the PLM.

% An overview of the recommendation framework is shown in Figure \ref{fig:fig1}. During inference time, candidate items are sorted by the output scores from the softmax layer. Accuracy of recommendation is defined as the hit ratio of the ground truth item within the top k sorted candidates.

% This approach doesn't necessarily depend on mentioned items to generate recommendations. By aligning dialog context with candidate items and learning similarities and discrepancies between item embeddings and dialog contexts, the \textbf{Ranking Encoder} is able to learn a meaningful mapping from item metadata to item embeddings. PLM is also able to harness this representation to make recommendations that are highly pertinent to dialog context through its multi-head attention mechanism. Experiments in section (\ref{sec:experiments}) show that the construction of item embeddings has positive contribution to the performance gain of recommendations.

\subsection{Dialog System}
Given a constructed dialog context $C$ from section \ref{sec:context}, we train the same PLM used above to reconstruct the current turn ground truth utterance (with item names replaced by the placeholder token) U = $(w_{0}, w_{1}, ..., w_{n})$. Only system utterances participate in training. The probability of generated response is formulated as:
\begin{align}
P(U | C) = \prod_{i=1}^{n} P(w_{i} | w_{i-1}, ..., w_{0}, C)
\end{align}
The loss function is set to be: 
\begin{align}
\label{loss:language}
L_{lang} = -\frac{1}{N} \sum_{i=1}^{N} log( P(U_i | C) )
\end{align}
where N is the number of utterances in a conversation. Note that both WTEs and ITEs exist in the constructed context. The inclusion of ITEs can help the PLM to generate placeholder tokens at the appropriate places and produce more diverse responses.

% During inference time, we append the top k ranked item vector embeddings to dialog history before generating system response, where k is a hyperparameter and defaulted to be 1. When we encounter a [PLACEHOLDER] token in generated responses, we replace this token with the item name of one of our recommended items by descending order of their ranking scores. Although our model doesn't require mentioned items to generate recommendations or system responses, experimental results show that incorporating mentioned items can boost recommendation accuracy.

Finally, we use the following loss to jointly train both the encoders and the language model:

\begin{align}
Loss = a \cdot L_{cg} + b \cdot  L_{cr} + c \cdot  L_{lang}
\end{align}
Where a, b and c are the weights of language training and recommendation training objectives, respectively. 

During inference, an embedding set over the entire item database is built with the \textbf{candidate encoder} and stored with nearest neighbor search indices. During response generation, when a [REC] token is generated, candidate generation \ref{sec:c_gen} is activated. An approximate nearest neighbor search is conducted on all embeddings stored and N candidates are selected based on their distances from the $O_{[REC]}$ vector. Candidate ranking is then activated and the PLM and \textbf{context encoder} are used to generate a score for each candidate. When ranking finishes, the ITE that receives the highest ranking score is appended to the dialog context and response generation continues until the end of sentence token is generated. 
